Efficient Progressive Image Compression with Variance-aware Masking

Learned progressive image compression is gaining momentum as it allows improved image reconstruction as more bits are decoded at the receiver. We propose a progressive image compression method in which an image is first represented as a pair of base-quality and top-quality latent representations. Next, a residual latent representation is encoded as the element-wise difference between the top and base representations. Our scheme enables progressive image compression with element-wise granularity by introducing a masking system that ranks each element of the residual latent representation from most to least important, dividing it into complementary components, which can be transmitted separately to the decoder in order to obtain different reconstruction quality. The masking system does not add further parameters nor complexity. At the receiver, any elements of the top latent representation excluded from the transmitted components can be independently replaced with the mean predicted by the hyperprior architecture, ensuring reliable reconstructions at any intermediate quality level. We also introduced Rate Enhancement Modules (REMs), which refine the estimation of entropy parameters using already decoded components. We obtain results competitive with state-of-the-art competitors, while significantly reducing computational complexity, decoding time, and number of parameters.

==> chapters/2_method/5_progressive_encdec.tex <==
\subsection{Progressive encoding and decoding}\label{prog}
Alg.~\ref{alg:encdec} details the encoding and the decoding phases for each slice $i$, when passing from a quality $\tilde{q}$ to an higher target quality $q^{*}$, with $q^{*} > \tilde{q}$.
Progressive encoding/decoding leverage $\sigma_{i}^{t}$ and $\mu_{i}^{t}$, whose values remain unchanged during the process.
%, in both the phases, we have at our disposable all the necessary information to reconstruct $\hat{y}_{i}^{q^*}$.
In lines 7-8 of Alg.~\ref{alg:encdec} we encode only the difference between $r_{i}^{q^*}$ and $r_{i}^{\tilde{q}}$, whereas all other values are masked. 
The masked elements are of two types: either they have already been encoded by the previous quality and don't need to be added to the bitstream again, or they belong to a higher quality and are replaced by the mean according to the masking policy described in sect. \ref{mask}.
 Since our method also allows us to know the positions of the elements encoded at quality $q^*$, during decoding it is possible to add them correctly to $\hat{r}_{i}^{\tilde{q}}$, already present in memory (line 11 of Alg.~\ref{alg:encdec}).



\begin{algorithm}
\caption{Encoding/Decoding  of the $i$-th slice at quality $q^{*}$  starting from  quality $\tilde{q}$}\label{alg:encdec}
\begin{algorithmic}[1]
\INPUT  \hspace{0.1cm} $q^{*}$, \hspace{0.05cm}  $\tilde{q}$, \hspace{0.05cm}, $\mu_{j}^{t}$, \hspace{0.05cm}$\sigma_{i}^{t}$, \hspace{0.05cm} $bs_{i}^{q^*}$ \text{if \textbf{decoding} else \textbf{None}}, \hspace{0.1cm}  $\hat{r}_{i}^{\tilde{q}}$ \text{if \textbf{decoding} else \textbf{None}}
\OUTPUT $bs_{i}^{q^*}$ \text{if \textbf{encoding} else }  $\hat{r}_{i}^{q^*}$
\State  $m_{i}^{\tilde{q}} \gets \mathcal{M}(\sigma_{i}^{t}, \tilde{q})$
\State  $m_{i}^{q^*} \gets \mathcal{M}(\sigma_{i}^{t}, q^*)$
\State  $m_{i}^{\Delta} \gets m_{i}^{q^*}  - m_{i}^{\tilde{q}}$
\State $\mu_{i}^{\Delta} \gets   \mu_{i}^{t}*m_{i}^{\Delta}$
\State $\sigma_{i}^{\Delta} \gets   \sigma_{i}^{t}*m_{i}^{\Delta}$ 
\If{\textbf{Encoding}}
    \State  $\hat{r}_{i}^{\Delta} \gets Round(r_{i}^{t} - \mu_{i}^{\Delta})\cdot \mu_{i}^{\Delta} $ 
    \State $bs_{i}^{\Delta}  \gets Encode(\hat{r}_{i}^{\Delta},\sigma_{i}^{\Delta} )$
\Else{}
     \State $\hat{r}_{i}^{\Delta} \gets Decode(bs_{i}^{\Delta},\sigma_{i}^{\Delta}) + \mu_{i}^{\Delta}$
     \State $\hat{r}_{i}^{q^*} \gets \hat{r}_{i}^{\tilde{q}}\cdot(1 - \mathcal{M}_{i}^{\Delta}) + \hat{r}_{i}^{\Delta}$ 
\EndIf


\end{algorithmic}
\end{algorithm}

==> chapters/5_additional_material/additional.tex <==


    


\section{Additional results }
\vspace{-0.5cm}
Fig. \ref{fig:mssim} compares our method with other progressive models regarding \emph{Multiscale  structural similarity index measure} (MS-SSIM) \cite{ssim} on Kodak. While slightly outperformed by Jeon overall, we maintain complexity improvements noted in the main manuscript.
Part of the future work will be to focus on perceptual metrics.
Fig. \ref{fig:mask_analysis} shows the distribution of the bpps against the quality of the reconstruction in terms of the mean squared error (MSE) when varying $q$.
As is evident, at lower bitrates, the length of the bitstream increases exponentially with the chosen percentile values $q$ used to generate progressive masks.
This trend is logical because initially we include points with higher standard deviations, which contain more information but require more bits for storage.
In contrast, as $q$ increases and approaches the maximum value (100), only points with a lower standard deviation are omitted, which however have minimal impact on the final bitstream.
Figures \ref{com_cpu} (a,b) show GFLOPs and the time to decode using a CPU on Kodak.



\begin{figure}[!h]
%\begin{minipage}[b]{1.0\linewidth} 
  \centering
 \includegraphics[width=0.65\columnwidth]{images/5_additional/results_mssm.pdf}
 % \vspace{0.1cm}
  \caption{bbp vs. MS-SSIM curve against existing progressive sotas models on Kodak: Proposed, Jeon, Lee, and JPEG2000. }
  \label{fig:mssim}
%\end{minipage}
\end{figure}

\begin{figure}[h!]
%\begin{minipage}[b]{1.0\linewidth} 
  \centering
 \includegraphics[width=0.60\columnwidth]{images/3_experiments/deltabppPercvsdist.pdf}
 % \vspace{0.1cm}
  \caption{Distribution of the bpps (orange) and MSE (green) when varying $q$ on Kodak.}
  \label{fig:mask_analysis}
%\end{minipage}
\end{figure}


\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=0.80\textwidth]{images/3_experiments/masking_policy/complexity_cpu_2.pdf}
        \subcaption{ }
        \label{fig:com1}
    \end{minipage}
    \vspace{-0.25cm}
    \begin{minipage}[b]{0.30\textwidth}
        \centering
        \includegraphics[width=0.80\textwidth]{images/3_experiments/masking_policy/timing_cpu_2.pdf}
        \subcaption{}
        \label{fig:com2}
    \end{minipage}
    \caption{GFLOPs and decoding time complexity on CPU (a,b)  vs.\ Jeon~\emph{et~al.}, considering different subranges on Kodak.}
    \label{com_cpu}
\end{figure}


\begin{figure*}[!b]
    \centering
    \begin{minipage}{0.8\textwidth}
        \centering
        % Riga 1
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim07/original.pdf}
            \subcaption{Input: bpp/PSNR/ \% of bpp}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim07/base.pdf}
            \subcaption{\emph{base}: 0.16/32.93/37}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim07/05.pdf}
            \subcaption{$q$=0.5:0.17/32.25/39.5}
        \end{minipage}
        
        \vspace{0.5cm} % Spazio tra le righe
        
        % Riga 2
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim07/kod_10.pdf}
            \subcaption{$q$=10:0.32/35.62/74}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim07/kod_25.pdf}
            \subcaption{$q$=25: 0.38/36.84/88 }
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim07/kod_100.pdf}
            \subcaption{$q$=10: 0.43/37.48/100}
        \end{minipage}
    \end{minipage}
    \caption{Reconstruction of Kodim07 from kodak dataset using proposed method.}
    \label{fig:kodim07}
\end{figure*}

Figures \ref{fig:kodim07},\ref{fig:kodim23} are  image reconstruction from Kodak.
Figures \ref{fig:main},\ref{fig:main2} are from CLIC validation dataset, with some latent representations across various qualities.







\begin{figure*}[]
    \centering
    \begin{minipage}{0.8\textwidth}
        \centering
        % Riga 1
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim23/or.pdf}
            \subcaption{Input: bpp/PSNR/ \% of bpp}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim23/base.pdf}
            \subcaption{\emph{base}: 0.096/33.33/34}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim23/kod_05.pdf}
            \subcaption{$q$=0.5:0.109/33.79/41.9}
        \end{minipage}
        
        \vspace{0.5cm} % Spazio tra le righe
        
        % Riga 2
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim23/kod_10.pdf}
            \subcaption{$q$=10:0.22/37.40/84.6}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim23/kod25.pdf}
            \subcaption{$q$=25: 0.24/37.89/92.3 }
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/kodim23/kod_100.pdf}
            \subcaption{$q$=10: 0.26/37.96/100}
        \end{minipage}
    \end{minipage}
    \caption{Reconstruction of Kodim23 from kodak dataset using proposed method.}
    \label{fig:kodim23}
\end{figure*}


\begin{comment}
    
\begin{figure*}[]
    \centering
    \begin{minipage}{0.8\textwidth}
        \centering
        % Riga 1
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0006/00006.png}
            \subcaption{Input: bpp/PSNR/ \% of bpp}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0006/base_0.24_28.77.png}
            \subcaption{\emph{base}: 0.24/28.77/33.8}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0006/q05_0.26_28.95.png}
            \subcaption{$q$=0.5:0.26/28.95/36.62}
        \end{minipage}
        
        \vspace{0.5cm} % Spazio tra le righe
        
        % Riga 2
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0006/q10_0.46_31.69.png}
            \subcaption{$q$=10:0.46/31.69/64.79}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0006/q25_0.65_34.23.png}
            \subcaption{$q$=25: 0.65/34.23/91.55 }
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0006/q10_0.71_34.8.png}
            \subcaption{$q$=10: 0.71/34.8/100}
        \end{minipage}
    \end{minipage}
    \caption{Reconstruction of 00006 from JPEG-AI dataset using proposed method.}
    \label{fig:jai6}
\end{figure*}




\begin{figure*}[]
    \centering
    \begin{minipage}{0.8\textwidth}
        \centering
        % Riga 1
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0013/00013_TE_1920x1280.png}
            \subcaption{Input: bpp/PSNR/ \% of bpp}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0013/base_0.21_30.32.png}
            \subcaption{\emph{base}: 0.21/30.32/36.8}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0013/q05_0.22_30.50.png}
            \subcaption{$q$=0.5:0.22/30.50/38.59}
        \end{minipage}
        
        \vspace{0.5cm} % Spazio tra le righe
        
        % Riga 2
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0013/q10_0.39_33.18_.png}
            \subcaption{$q$=10:0.39/33.18/68.4}
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0013/q25_0.53_35.08.png}
            \subcaption{$q$=25: 0.53/35.083/92.98 }
        \end{minipage}\hfill
        \begin{minipage}{0.3\textwidth}
            \centering
            \includegraphics[width=\linewidth]{images/5_additional/0013/q100_0.57_35.51.png}
            \subcaption{$q$=10: 0.57/35.51/100}
        \end{minipage}
    \end{minipage}
    \caption{Reconstruction of a sample from JPEG-AI dataset using our proposed method.}
    \label{fig:jai13}
\end{figure*}

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%% LATENTS 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!h]
    \centering
    \begin{minipage}[t]{0.7\textwidth}
        \centering
        % Big image
        \includegraphics[width=1\textwidth]{images/5_additional/schika/or/input.pdf}
        \subcaption{Input image}
        \vfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/base/std_base_258.png}
            \subcaption{Base std}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/base/ch_base_258.png}
            \subcaption{Base channel}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/base/crop_0.08_34.21.png}
            \subcaption{Rec. (0.08,34.14)}
        \end{minipage}




    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.7\textwidth}
        \centering
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/0.5/mask_0.05_258.png}
            \subcaption{mask at $q$=0.5}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/0.5/std_0.05_258.png}
            \subcaption{std at $q$=0.5}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/0.5/ch_0.05_258.png}
            \subcaption{channel at $q$=0.5}
        \end{minipage}
        \hfill 
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/0.5/crop_0.09_34.54.png}
            \subcaption{Rec (0.09,34.54)}
        \end{minipage}
        \hfill

        
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/7.5/mask_0.5_258.png}
            \subcaption{mask at $q$=7.5}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/7.5/std_0.5_258.png}
            \subcaption{std at $q$=7.5}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/7.5/ch_0.5_258.png}
            \subcaption{channel at $q$=7.5}
        \end{minipage}
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/7.5/crop_0.18_37.15.png}
            \subcaption{Rec. (0.18,37.15)}
        \end{minipage}

        \vfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/20/l_20_258.png}
            \subcaption{Mask at $q$=20}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/20/std_20_258.png}
            \subcaption{std at $q$=20}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/20/ch_20_258.png}
            \subcaption{channel at $q$=20}
        \end{minipage}
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/20/crop_0.21_38.04.png}
            \subcaption{Rec. (0.21,38.04)}
        \end{minipage}
        \vfill

        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/100/ch_10_258.png}
            \subcaption{Std at $q$=100 (top).}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/100/tl_10_258.png}
            \subcaption{channel at $q$=100 (top)}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/schika/100/crop_0.23_38.30.png}
            \subcaption{Rec. (0.23,38.3)}
        \end{minipage}
    \end{minipage}
    \caption{Final reconstruction with latent representations for different qualities, which varies through the raws.}\label{fig:main}
\end{figure*}




%%%%%%%%%%%%%%%%%%%%%%% LATENTS 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!h]
    \centering
    \begin{minipage}[t]{0.7\textwidth}
        \centering
        % Big image
        \includegraphics[width=1\textwidth]{images/5_additional/roberto/or/input_rob.pdf}
        \subcaption{Input image}
        \vfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/or/std_base_258.png}
            \subcaption{Base std}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/or/ch_base_258.png}
            \subcaption{Base channel}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/base/crop_0.05_35.45.png}
            \subcaption{Rec. (0.05,35.45)}
        \end{minipage}




    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.7\textwidth}
        \centering
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/0.5/m_0.05_258.png}
            \subcaption{mask at $q$=0.5}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/0.5/ch_0.05_258.png}
            \subcaption{std at $q$=0.5}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/0.5/tl_0.05_258.png}
            \subcaption{channel at $q$=0.5}
        \end{minipage}
        \hfill 
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/0.5/crop_0.06_35.92.png}
            \subcaption{Rec (0.06,35.92)}
        \end{minipage}
        \hfill

        
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/10/mask_1_258.png}
            \subcaption{mask at $q$=10}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/10/ch_1_258.png}
            \subcaption{std at $q$=10}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/10/ch_1_258.png}
            \subcaption{channel at $q$=10}
        \end{minipage}
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/10/crop_0.13_38.81.png}
            \subcaption{Rec. (0.13,38.81)}
        \end{minipage}

        \vfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/15/l_1.5_258.png}
            \subcaption{Mask at $q$=15}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/15/std_1.5_258.png}
            \subcaption{std at $q$=15}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/15/ch_1.5_258.png}
            \subcaption{channel at $q$=15}
        \end{minipage}
        \begin{minipage}[t]{0.24\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/15/crop_0.14_38.86.png}
            \subcaption{Rec. (0.14,38.86)}
        \end{minipage}
        \vfill

        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/100/std_10_258.png}
            \subcaption{Std at $q$=100 (top).}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/100/ch_10_258.png}
            \subcaption{channel at $q$=100 (top)}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.3\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/5_additional/roberto/100/crop_0.142_38.886.png}
            \subcaption{Rec. (0.142,38.88)}
        \end{minipage}
    \end{minipage}
    \caption{Final reconstruction with latent representations for different qualities, which varies through the raws.}\label{fig:main2}
\end{figure*}
